Towards Hardware Support for FPGA Resource Elasticity

FPGAs are increasingly being deployed in the cloud to accelerate diverse applications. They are to be shared among multiple tenants to improve the total cost of ownership. Partial reconfiguration technology enables multi-tenancy on FPGA by partitioning it into regions, each hosting a specific application's accelerator. However, the region's size can not be changed once they are defined, resulting in the underutilization of FPGA resources. This paper argues to divide the acceleration requirements of an application into multiple small computation modules. The devised FPGA shell can reconfigure the available PR regions with those modules and enable them to communicate with each other over Crossbar interconnect with the Wishbone bus interface. For each PR region being reconfigured, it updates the register file with the valid destination addresses and the bandwidth allocation of the interconnect. Any invalid communication request originating from the Wishbone master interface is masked in the corresponding master port of the crossbar. The allocated bandwidth for the PR region is ensured by the weighted round-robin arbiter in the slave port of the crossbar. Finally, the envisioned resource manager can increase or decrease the number of PR regions allocated to an application based on its acceleration requirements and PR regions' availability.

==> sections/ack.tex <==
\section*{Acknowledgments}
We would like to thank colleagues at Ericsson Research supporting this work and giving feedback on the draft of the paper.
